Faster Configuration Performance Bug Testing with Neural Dual-level Prioritization

As software systems become more complex and configurable, more performance problems tend to arise from the configuration designs. This has caused some configuration options to unexpectedly degrade performance which deviates from their original expectations designed by the developers. Such discrepancies, namely configuration performance bugs (CPBugs), are devastating and can be deeply hidden in the source code. Yet, efficiently testing CPBugs is difficult, not only due to the test oracle is hard to set, but also because the configuration measurement is expensive and there are simply too many possible configurations to test. As such, existing testing tools suffer from lengthy runtime or have been ineffective in detecting CPBugs when the budget is limited, compounded by inaccurate test oracle. In this paper, we seek to achieve significantly faster CPBug testing by neurally prioritizing the testing at both the configuration option and value range levels with automated oracle estimation. Our proposed tool, dubbed NDP, is a general framework that works with different heuristic generators. The idea is to leverage two neural language models: one to estimate the CPBug types that serve as the oracle while, more vitally, the other to infer the probabilities of an option being CPBug-related, based on which the options and the value ranges to be searched can be prioritized. Experiments on several widely-used systems of different versions reveal that NDP can, in general, better predict CPBug type in 87% cases and find more CPBugs with up to 88.88x testing efficiency speedup over the state-of-the-art tools.

==> Background-old.tex <==
\section{Background}

\subsection{The Discovery and Exploration of CPBugs}
Performance bugs are closely related to software configurability. Jin et al. and Han et al.[1,2] found that most performance issues (59\%) in large-scale software systems are related to configuration problems, leading to a high prevalence of CPBugs in modern software systems. Xiang et al. [13] suggest using configuration option documentation, which describes the names, functions, and usage of configuration options, as a good source for deriving configuration-related performance properties, as they are widely available and easy to obtain. Therefore, our target systems are large-scale software systems with detailed and standardized configuration option documentation. By analyzing different versions of the software and their configuration option documentation over long-term iterations, we can extract performance-related configuration properties to help identify potential CPBugs.

Existing debugging techniques can only detect performance bugs with known patterns. Nistor et al. [3,4,5,6,7] used inefficient code patterns as test oracles, which can identify loops with inefficient memory access patterns, indicating potential performance bugs. While effective in some scenarios, this method's limitation lies in its ability to identify only predefined inefficient patterns, failing to cover all types of performance issues. Coppa et al. [8] proposed analysis-based techniques to detect performance bottlenecks that may cause significant slowdowns. However, because some slowdown behaviors may spontaneously arise from intensive computation, determining whether these slowdowns are performance bugs becomes difficult. Therefore, these analysis-based methods may not always accurately identify performance issues in complex and dynamically changing systems. The oracles in the aforementioned studies can only detect performance bugs with fixed patterns, which are not applicable to many real-world CPBugs we study. The complexity and diversity of CPBugs mean they often cannot be identified through simple pattern matching. The configuration options in modern software systems are diverse, and different configuration combinations may lead to different performance outcomes, requiring more flexible and intelligent detection methods.

Ying et al. [23] discussed the nature of Configuration-Triggered Bugs (CTBug) through empirical studies, analyzing key configurations in fault reports with the help of large language models, which aids in reproducing some CPBugs. Shen et al. [9] proposed a heuristic search-based testing framework to search software inputs for potential performance bottlenecks. This provides us with some ideas; combining heuristic algorithms, we can often quickly obtain configuration pairs with the greatest performance differences, allowing us to expose CPBugs more rapidly. Jamshidi et al. [10] proposed configuration performance modeling, and Nair et al. [11] proposed configuration-based performance tuning. The former aims to predict the performance of a given configuration, while the latter studies the trend of performance changes when adjusting configurations and finds the optimal configuration in terms of performance. Wang et al. [29] further studied the system's reactions to different configurations. This type of research provides ideas and directions for summarizing performance-related configuration properties. Specifically, we can use data-driven methods to understand and judge system performance, discovering abnormal configuration options and exposing CPBugs through detailed analysis of system behavior under different configurations.

\subsection{Related Work}
In recent years, work on software configuration testing and performance testing has been steadily advancing. Gargantini et al. [20] proposed four new combinatorial testing strategies to generate test cases, exposing various potential configuration faults by comparing the expected responses of configuration settings with the actual system performance. Shuai et al. [21] proposed unified regression test selection (URTS) to conduct different configuration tests across different software versions, significantly reducing the number of tests by skipping equivalent tests and efficiently identifying potential constraints and misconfigurations. Junqiang et al. [22] performed configuration fuzz testing on software based on known configuration constraint relationships, using heuristic methods to intelligently mutate parameter sets with dependencies and constraints, filtering out configuration parameters unlikely to cause errors. Han et al. [31] generated a configuration performance testing framework based on constraint and strength files, limiting the number of parameters tested, the intensity of interactions, and ensuring the validity of parameter combinations. These research results enhance the efficiency and accuracy of software configuration testing by filtering configuration performance testing parameters from different angles.

Reusing different types of tests can greatly accelerate testing efficiency. Zishuo et al. [32] conducted performance tests using existing tests in the software release pipeline, revealing performance changes before and after software upgrades. Xudong et al. [33] transformed unit tests and other test cases of software systems into configuration tests, avoiding repetitive work by testers during configuration performance testing.

Performance testing can often be very time-consuming. AlGhamdi et al. [24,25] used statistical tests during performance testing to determine whether data from multiple time periods have statistically significant differences and dynamically detect system operation status during testing to decide when to stop performance testing. Simin et al. [30] used hardware-independent metrics to replace hardware-dependent performance metrics, reducing performance testing errors and events. These approaches help testers effectively shorten performance testing time, aligning with the characteristics of the DevOps era.

==> Understanding_CPBugs.tex <==
\section{UNDERSTANDING CPBUGS}

\subsection{CPBugs Oracle}
\textbf{Finding 1:} Most (87.6\%) CPBugs exhibit unexpected performance changes when adjusting configuration options. This result indicates that performance expectations can serve as an effective oracle for exposing CPBugs [18]. 

For each option, we can use the expected performance changes of different values of configuration options as performance Properties to expose CPBugs by detecting attribute violations. To evaluate the extent to which the attribute-based approach can expose CPBugs, Haochen, H et al. studied the prevalence of unexpected performance changes when adjusting the configuration options of CPBugs. They manually studied all 173 collected CPBugs and found that 150 (86.7\%) exhibited unexpected performance changes when adjusting configuration options. This result indicates that performance expectations can serve as an effective oracle for exposing CPBugs. The remaining 23 (13.3\%) CPBugs could not be exposed mainly due to inconsistent expectations of configuration options, with some configuration options lacking common expected performance changes.

Thus, the determination of CPBug mainly involves comparing the expected performance of the configuration (e.g., throughput, latency, execution time) with the actual impact of the configuration on performance. A mismatch between the expected and actual performance changes usually indicates the presence of a CPBug [18]. Specifically, there are two scenarios:
\begin{itemize}
\item The direction of expected and actual performance chan-ges is different.
\item The direction of expected and actual changes is the same, but the magnitude of the changes does not meet expectations.
\end{itemize}

For scenario 1, there are usually different performance trends from the expected trend, which implies that there is a significant issue in some code segments of the configuration option, leading to completely different performance directions. As shown in Figure 1, it depicts a real CPBug related to the \verb|read_buffer_size| configuration option in MySQL, including its fault description and fix method. This option is mainly used to change the size of the read buffer allocated for each sequential table scan request. In our expectation, increasing this option value should allow MySQL to cache more results, so a larger buffer should improve performance. However, performance dropped when increasing the value beyond 256K. This is because \verb|MyISAM| initializes an \verb|IO_CACHE| for writing and uses \verb|read_buffer_size| for bulk inserts. \verb|my_malloc| is called with the \verb|MY_ZEROFILL| flag, which causes \verb|memset| to be called on the size of \verb|read_buffer_size|, resulting in relatively large performance decreases.

Scenario 2 is relatively more complex; we need to find a series of thresholds to indicate abnormal performance change magnitudes. Haochen, H et al. adopted the following rules to determine whether the degree of change exceeded expectations:

\begin{align}
P(V_{src})/P(V_{tar})>T_{r_{1}}
\end{align}
\begin{align}
P(V_{src})-P(V_{tar})>T_{r_{2}}
\end{align}
\\
Where Tr1 and Tr2 are predefined thresholds. This means P(Vsrc) is better than P(Vtar) by more than Tr1 times. And the absolute decrease from P(Vsrc) to P(Vtar) is greater than Tr2. According to Figure 2, the authors finally obtained the optimal combination of Tr1 and Tr2 as 3 and 5 (the peaks of the blue line) through the successfully replicated data of 41 CPBugs.

\begin{figure}[htbp]
\centerline{\includegraphics[width=\linewidth]{fig/图片 1.png}}
\caption{A real-world CPBug.\textit{The incorrect use of a flag in the program results in a call to memset based on the size of read\_buffer\_size.}}
\label{fig}
\end{figure}

\begin{figure}[htbp]
\centerline{\includegraphics[width=\linewidth]{fig/图片 2.png}}
\caption{ F-score values reflected by different Tr1 and Tr2}
\label{fig}
\end{figure}

\subsection{performance Properties in CPBugs}

\textbf{Finding 2:} Most (87.6\%) configuration options that have triggered CPBugs exhibit expected performance changes that are relatively simple and intuitive. Some options have the same performance change trends, that is, the same performance properties.

Haochen et al. studied 150 CPBugs to understand the performance properties of misconfigured options. Through manual analysis, they summarized five semantic types: optimization switches, non-functional trade-offs, resource allocation, functional switches, and non-impact options, as shown in Table 1. Specifically, they have the following properties:

\begin{itemize}
\item\textbf{Optimization Switch:} When enabled, an optimization strategy is activated, and performance is expected to improve. However, if the actual performance degrades, a potential CPBug is present.
\item\textbf{Non-functional Trade-off:} (such as ACID properties, used to maintain consistency and correctness): Configuration options are used to balance the program's performance and other non-functional requirements. Adjusting the configuration values to relax constraints is expected to enhance performance.
\item\textbf{Resource Allocation:} Used to control resource usage, allocating more resources is generally expected to bring better performance.
\item\textbf{Functional Switch:} Configuration options control non-performance functionalities but indirectly affect the system's performance. When an option disables a function, system performance usually improves.
\item\textbf{Non-impact Option:} These configuration options should not affect the system's performance, i.e., performance is expected to remain unchanged after adjusting the options.
\end{itemize}

Table 1 broadly categorizes the expected performance of configuration options. If correctly classified, the presence of a CPBug can be quickly identified by comparing the expected and actual performance changes. However, misclassification and uncommon expected performance changes might lead to false positives. In such cases, we can increase the number of sampling tests to observe if multiple types of performance tendencies appear within the sampling range of the configuration options (see Section 4). It also shows that unexpected changes usually occur in non-functional trade-offs and functional switches. Of course, optimization switches and resource allocation might also appear (not observed in the 150 CPBugs studied by Haochen et al.).

Haochen et al. used natural language processing and association rule mining methods for classification. Specifically, they first divided manual configuration descriptions into multiple sentences of the same configuration type, then normalized the words in each sentence from syntactic and semantic aspects. They then mined specific and frequently occurring word sequences in the descriptions of specific configuration types. After selecting the best rules, these rules were used for voting classification. All matching description rules would vote for their corresponding types, and the type with the highest weight was selected as the configuration type. In the improved scheme, natural language processing models (such as BERT and RoBERTa) under the transformer framework were used for text classification, yielding good preliminary results (see Section 4).

\begin{table*}
\caption{Performance Properties in CPBugs.}
    \centering
    \begin{tabular}{@{}c@{\;}c@{}} % 使用 m{0.5cm} 来创建列间距
        \includegraphics[width=\linewidth]{fig/表格 1.png} 
    \end{tabular}
    \label{tab:my_table}
\end{table*}
    




\subsection{Problems with numerical CPBugs}

To conduct software testing through the performance properties of configuration options, we sample at least two values in one test. However, due to the vast possible values of numerical options (mainly resource allocation options), it is difficult to enumerate all value pairs. Therefore, Haochen et al. manually reproduced the value ranges of 26 out of 37 numerical CPBugs studied. Some values can reach the 64-bit computer encoding limit or even more. Due to the limitations of experimental resources (such as CPU cores and memory) and the potential extreme boundary effects, we decided to limit the upper bounds of these numerical options to the acceptable range of experimental resources.

\textbf{Finding 3: }96.1\% of numeric configuration options trigger CPBugs when set to their minimum or maximum values [18].

As shown in Figure 3, 25 out of the 26 numerical options have CPBug triggering ranges that include the maximum or minimum values. The reason is that within a reasonable value range, most values of numerical options significantly impact data flow, but they usually do not change control flow. In other words, conventional changes in numerical configuration options typically only adjust the state of existing software paths, such as alleviating or amplifying effects, and rarely trigger new execution paths.

\textbf{Finding 4: }92.3\% of numerical configuration options trigger CPBugs when set to middle values.

Furthermore, we found that in these 26 numerical configuration options, 24 have CPBug triggering ranges located in the middle of the value range. This pattern indicates that although conventional values of numerical options have limited impact on control flow, they can significantly affect software behavior at certain critical values. These critical values may touch upon sensitive conditions or boundary situations in software design, thereby altering control flow.

Moreover, even among options that can trigger errors, we observed continuity and extensiveness in CPBug triggering ranges. These ranges are often continuous large segments and include many common values. This may be because the software behavior near these values is more susceptible to the influence of configuration options, thereby increasing the likelihood of triggering errors.

\begin{figure}[htbp]
\centerline{\includegraphics[width=\linewidth]{fig/new_fig3.png}}
\caption{Value ranges that can trigger CPBugs (dark gray).}
\label{fig}
\end{figure}

==> table/new-software.tex <==
\begin{table}[t!]
\centering

\setlength{\tabcolsep}{1mm}
\caption{Configurable software with CPBugs.}

\label{tb:software}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{lllllll}
 \toprule

\textbf{Software} & \textbf{$\#$CPBugs} & \textbf{$\#$Type-1} & \textbf{$\#$Type-2} & \textbf{$\#$Type-3} & \textbf{$\#$Type-4} & \textbf{$\#$Type-5}  \\

\midrule



 \bottomrule
\end{tabular}
}
\end{table}


==> table/rq2.tex <==
\begin{table}[t!]
%\caption{\revision{The best efficiency of each approach by computing how many tested options/much clock time is required to find per CPBug.}}
\caption{\revision{The least tested options/clock time required to find per CPBug by each approach.}}
\label{tb:rq2}
\centering
\begin{tabular}{llll|lll}
\hline
\toprule
\multirow{2}{*}{\textbf{System}}&\multicolumn{3}{c|}{\textbf{$\#$ Tested Options}}&\multicolumn{3}{c}{\textbf{Time (min)}}\\

\cmidrule{2-7}

&\approach&\texttt{CPD}&\texttt{KS}&\approach&\texttt{CPD}&\texttt{KS}\\

\midrule

MySQL & 1.6 & 5.1 & 5.1 & 120.0 & 380.2 & 380.2 \\
MariaDB & 6.0 & 12.7 & 12.7  & 153.4 & 324.7 & 324.7 \\
Apache & 12.0 & 30.3 & 30.3  & 536.2 & 1351.6 & 1351.6 \\
Gcc & 2.1 & 2.5 & 2.3  & 18.0 & 21.0 & 19.4 \\
Clang & 3.0 & 5.5 & 6.3  & 25.2 & 46.2 & 53.2 \\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table}

==> table/rq3.tex <==
\begin{table}[t!]
%\caption{\revision{The best efficiency of each approach by computing how many test counts/much clock time is required to find per CPBug on numeric options.}}
\caption{\revision{The least test counts/clock time required to find per CPBug on numeric options by each approach.}}
\label{tb:rq3}
\centering
\footnotesize
\begin{tabular}{llll|lll}
\hline

\toprule
\multirow{2}{*}{\textbf{System}}&\multicolumn{3}{c|}{\textbf{$\#$ Test Counts}}&\multicolumn{3}{c}{\textbf{Time (min)}}\\

\cmidrule{2-7}

&\approach&\texttt{CPD}&\texttt{KS}&\approach&\texttt{CPD}&\texttt{KS}\\

\midrule


MySQL & 1.0 & 7.6 & 88.8 & 4.9 & 37.0 & 432.4 \\
MariaDB & 1.0 & 2.5 & 23.0 & 1.7 & 4.25 & 39.1 \\
Apache & 1.0 & 10.5 & 52.0 & 4.2 & 44.1 & 218.4 \\

\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table}

==> table/rq4-bk.tex <==
\begin{table}
\caption{New CPBugs detected by NDP.}
\label{tb:rq4}
\centering
\begin{tabular}{l|l|l}
\toprule
CPBug & Slowdown & CPBug Type \\
\midrule
-O1 & 1.59x Compiling Time & Type-1 \\

-O2 & 1.34x Compiling Time & Type-1 \\

-Og & 1.40x Compiling Time & Type-1 \\

-Ofast & 1.64x Compiling Time & Type-1 \\

-fno-asm & 1.11x Compiling Time & Type-4 \\

-floop-interchange & 1.14x Compiling Time & Type-1 \\
-ffloat-store & 1.12x Compiling Time & Type-4 \\

-Ofast & 1.13x Execution Time & Type-1 \\
-O2 & 1.18x Execution Time & Type-1 \\
 \bottomrule
\end{tabular}
\label{table:options}
\end{table}
% \begin{table*}[t!]
% \caption{Effectiveness of estimating CPBugs types.}
% \label{tb:rq4}
% %\setlength{\tabcolsep}{0.6mm}
% \centering
% \footnotesize
% \begin{tabular}{lllll|lll|lll}


% \toprule


% \multirow{2}{*}{\textbf{Option}}&\multirow{2}{*}{\textbf{Options}}&\multicolumn{3}{c|}{\textbf{Option value pairs}}&\multicolumn{3}{c|}{\textbf{Special option value pairs}}&\multicolumn{3}{c}{\textbf{CPBug trigger probability



% }}\\

% \cmidrule{3-11}

% &&\approach&\texttt{CP-Detector}&\texttt{Baseline}&\approach&\texttt{CP-Detector}&\texttt{Baseline}&\approach&\texttt{CP-Detector}&\texttt{Baseline}\\

% \midrule

% innodb_log_file_size&Optimization&4&19&190&4&5&75&100\%&26.31\%&39.47\%\\

% innodb_buffer_pool_size&Tradeoff&10&45&1035&10&31&465&100\%&68.89\%&44.93\%\\

% virtualhost&Resource&1&15&120&1&5&93.2&100\%&33.33\%&45.83\%\\



% %\textsc{Trimesh}&Mesh&\textsc{O1:} \# Iteration; \textsc{O2:} Latency&13&239,260\\

% %&\makecell[l]{Latency\\Throughput}&3&1,343&\makecell[l]{Apache Storm under the Word \\Count on OpenNebula(1 CPU)}\\



% %1.92$\times 10^{10}$

% \bottomrule
% \end{tabular}
% %}
% %\centering
% % \begin{tablenotes}
% %    \footnotesize
% %    %\item The configuration options are preprocessed and thus only the ones (and their ranges) that can affect the performance attributes are considered. 
% %    \item $\lvert \mathbfcal{O} \rvert$ denotes number of options. We run all systems under their standard benchmarks. More details can be found at: \href{https://github.com/taochen/mmo-fse-2021}{\texttt{\textcolor{blue}{https://github.com/taochen/mmo-fse-2021}}}.
% %    \end{tablenotes}
%     % Notably, \textsc{Storm} and \textsc{Keras-DNN} have three benchmarks and two dataset, respectively.
% \end{table*}

==> table/rq4.tex <==
\begin{table}[t!]
\caption{\revision{New CPBugs discovered by NDP.}}
\label{tb:rq4}
\centering
\begin{tabular}{l|l|l}
\toprule
CPBug & Slowdown & CPBug Type \\
\midrule
-O1 & 1.59x Compiling Time & Type-1 \\

-O2 & 1.34x Compiling Time & Type-1 \\

-Og & 1.40x Compiling Time & Type-1 \\

-Ofast & 1.64x Compiling Time & Type-1 \\

-fno-asm & 1.11x Compiling Time & Type-4 \\

-floop-interchange & 1.14x Compiling Time & Type-1 \\
-ffloat-store & 1.12x Compiling Time & Type-4 \\

-Ofast & 1.13x Execution Time & Type-1 \\
-O2 & 1.18x Execution Time & Type-1 \\
 \bottomrule
\end{tabular}

\vspace{-0.2cm}
\end{table}
% \begin{table*}[t!]
% \caption{Effectiveness of estimating CPBugs types.}
% \label{tb:rq4}
% %\setlength{\tabcolsep}{0.6mm}
% \centering
% \footnotesize
% \begin{tabular}{lllll|lll|lll}


% \toprule


% \multirow{2}{*}{\textbf{Option}}&\multirow{2}{*}{\textbf{Options}}&\multicolumn{3}{c|}{\textbf{Option value pairs}}&\multicolumn{3}{c|}{\textbf{Special option value pairs}}&\multicolumn{3}{c}{\textbf{CPBug trigger probability



% }}\\

% \cmidrule{3-11}

% &&\approach&\texttt{CP-Detector}&\texttt{Baseline}&\approach&\texttt{CP-Detector}&\texttt{Baseline}&\approach&\texttt{CP-Detector}&\texttt{Baseline}\\

% \midrule

% innodb_log_file_size&Optimization&4&19&190&4&5&75&100\%&26.31\%&39.47\%\\

% innodb_buffer_pool_size&Tradeoff&10&45&1035&10&31&465&100\%&68.89\%&44.93\%\\

% virtualhost&Resource&1&15&120&1&5&93.2&100\%&33.33\%&45.83\%\\



% %\textsc{Trimesh}&Mesh&\textsc{O1:} \# Iteration; \textsc{O2:} Latency&13&239,260\\

% %&\makecell[l]{Latency\\Throughput}&3&1,343&\makecell[l]{Apache Storm under the Word \\Count on OpenNebula(1 CPU)}\\



% %1.92$\times 10^{10}$

% \bottomrule
% \end{tabular}
% %}
% %\centering
% % \begin{tablenotes}
% %    \footnotesize
% %    %\item The configuration options are preprocessed and thus only the ones (and their ranges) that can affect the performance attributes are considered. 
% %    \item $\lvert \mathbfcal{O} \rvert$ denotes number of options. We run all systems under their standard benchmarks. More details can be found at: \href{https://github.com/taochen/mmo-fse-2021}{\texttt{\textcolor{blue}{https://github.com/taochen/mmo-fse-2021}}}.
% %    \end{tablenotes}
%     % Notably, \textsc{Storm} and \textsc{Keras-DNN} have three benchmarks and two dataset, respectively.
% \end{table*}

==> table/software-bk.tex <==
\begin{table}[t!]
\centering

\setlength{\tabcolsep}{1mm}
\caption{Configurable software with CPBugs.}

\label{tb:software}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{lll}
 \toprule

\textbf{Software} & \textbf{$\#$CPBugs} & \textbf{CPBugs Distribution with respect to Types}  \\

\midrule
\textsc{MySQL} & 30 & Type-1=8; Type-2=6; Type-3=8; Type-4=6; Type-5=1\\
\textsc{MariaDB} & 10 & Type-1=3; Type-2=0; Type-3=4; Type-4=2; Type-5=1\\
\textsc{Apache} & 5 & Type-1=0; Type-2=1; Type-3=1; Type-4=1; Type-5=1\\
\textsc{Gcc} & 15 & Type-1=1; Type-2=10; Type-3=0; Type-4=2; Type-5=2\\
\textsc{Clang} & 6 & Type-1=0; Type-2=6; Type-3=0; Type-4=0; Type-5=0  \\


 \bottomrule
\end{tabular}
}
\end{table}

